Spectral partitioning in equitable graphs

Graph partitioning problems emerge in a wide variety of complex systems, ranging from biology to finance, but can be rigorously analyzed and solved only for a few graph ensembles. Here, an ensemble of equitable graphs, i.e. random graphs with a block-regular structure, is studied, for which analytical results can be obtained. In particular, the spectral density of this ensemble is computed exactly for a modular and bipartite structure. Kesten-McKay's law for random regular graphs is found analytically to apply also for modular and bipartite structures when blocks are homogeneous. Exact solution to graph partitioning for two equal-sized communities is proposed and verified numerically, and a conjecture on the absence of an efficient recovery detectability transition in equitable graphs is suggested. Final discussion summarizes results and outlines their relevance for the solution of graph partitioning problems in other graph ensembles, in particular for the study of detectability thresholds and resolution limits in stochastic block models.

==> bibSpectra.tex <==
\bibitem{blondel2008fast}Blondel, Vincent D., et al. "Fast unfolding of communities in large networks." Journal of statistical mechanics: theory and experiment 2008.10 (2008): P10008.

\bibitem{bollobas1999exact}Bollob‡s, BŽla, and Alex D. Scott. "Exact bounds for judicious partitions of graphs." Combinatorica 19.4 (1999): 473-486.

\bibitem{mezard2002analytic}MŽzard, Marc, Giorgio Parisi, and Riccardo Zecchina. "Analytic and algorithmic solution of random satisfiability problems." Science 297.5582 (2002): 812-815.

\bibitem{barucca2016centrality}Barucca, Paolo, Daniele Tantari, and Fabrizio Lillo. "Centrality metrics and localization in core-periphery networks." Journal of Statistical Mechanics: Theory and Experiment 2016.2 (2016): 023401.

\bibitem{barucca2016disentangling}Barucca, Paolo, and Fabrizio Lillo. "Disentangling bipartite and core-periphery structure in financial networks." Chaos, Solitons & Fractals 88 (2016): 244-253.

\bibitem{easley2010networks}Easley, David, and Jon Kleinberg. Networks, crowds, and markets: Reasoning about a highly connected world. Cambridge University Press, 2010.

\bibitem{holland1983stochastic}Holland, Paul W., Kathryn Blackmond Laskey, and Samuel Leinhardt. "Stochastic blockmodels: First steps." Social networks 5.2 (1983): 109-137.

\bibitem{mossel2013proof}Mossel, Elchanan, Joe Neeman, and Allan Sly. "A proof of the block model threshold conjecture." arXiv preprint arXiv:1311.4115 (2013).

\bibitem{caldarelli2002scalefree}Caldarelli, Guido, et al. "Scale-free networks from varying vertex intrinsic fitness." Physical review letters 89.25 (2002): 258702.

\bibitem{bianconi2013statistical}Bianconi, Ginestra. "Statistical mechanics of multiplex networks: Entropy and overlap." Physical Review E 87.6 (2013): 062806.

\bibitem{garlaschelli2008maximum}Garlaschelli, Diego, and Maria I. Loffredo. "Maximum likelihood: Extracting unbiased information from complex networks." Physical Review E 78.1 (2008): 015101.

\bibitem{robins2007introduction}Robins, Garry, et al. "An introduction to exponential random graph (p*) models for social networks." Social networks 29.2 (2007): 173-191.

\bibitem{larremore2014efficiently}Larremore, Daniel B., Aaron Clauset, and Abigail Z. Jacobs. "Efficiently inferring community structure in bipartite networks." Physical Review E 90.1 (2014): 012805.

\bibitem{hendrickson1995improved}Hendrickson, Bruce, and Robert Leland. "An improved spectral graph partitioning algorithm for mapping parallel computations." SIAM Journal on Scientific Computing 16.2 (1995): 452-469.

\bibitem{strogatz2001exploring}Strogatz, Steven H. "Exploring complex networks." Nature 410.6825 (2001): 268-276.

\bibitem{hidalgo2009building}Hidalgo, CŽsar A., and Ricardo Hausmann. "The building blocks of economic complexity." proceedings of the national academy of sciences 106.26 (2009): 10570-10575.

\bibitem{newman2002random}Newman, Mark EJ, Duncan J. Watts, and Steven H. Strogatz. "Random graph models of social networks." Proceedings of the National Academy of Sciences 99.suppl 1 (2002): 2566-2572.

\bibitem{rogers2008cavity}Rogers, Tim, et al. "Cavity approach to the spectral density of sparse symmetric random matrices." Physical Review E 78.3 (2008): 031116.

\bibitem{reed2004finding}Reed, Bruce, Kaleigh Smith, and Adrian Vetta. "Finding odd cycle transversals." Operations Research Letters 32.4 (2004): 299-301.

\bibitem{rogers2009cavity}Rogers, Tim, and Isaac PŽrez Castillo. "Cavity approach to the spectral density of non-Hermitian sparse matrices." Physical Review E 79.1 (2009): 012101.

\bibitem{karypis1999fast}Karypis, George, and Vipin Kumar. "A fast and high quality multilevel scheme for partitioning irregular graphs." SIAM Journal on scientific Computing 20.1 (1998): 359-392.

\bibitem{pothen1990partitioning}Pothen, Alex, Horst D. Simon, and Kang-Pu Liou. "Partitioning sparse matrices with eigenvectors of graphs." SIAM journal on matrix analysis and applications 11.3 (1990): 430-452.

\bibitem{boppana1987eigenvalues}Boppana, Ravi B. "Eigenvalues and graph bisection: An average-case analysis." Foundations of Computer Science, 1987., 28th Annual Symposium on. IEEE, 1987.

\bibitem{zdeborova2010conjecture}Zdeborov‡, Lenka, and Stefan Boettcher. "A conjecture on the maximum cut and bisection width in random regular graphs." Journal of Statistical Mechanics: Theory and Experiment 2010.02 (2010): P02020.

\bibitem{fricke2015coreperiphery}Fricke, Daniel, and Thomas Lux. "CoreÐperiphery structure in the overnight money market: evidence from the e-mid trading platform." Computational Economics 45.3 (2015): 359-395.

\bibitem{smith1992structure}Smith, David A., and Douglas R. White. "Structure and dynamics of the global economy: network analysis of international trade 1965Ð1980." Social forces 70.4 (1992): 857-893.

\bibitem{fortunato2007resolution}Fortunato, Santo, and Marc Barthelemy. "Resolution limit in community detection." Proceedings of the National Academy of Sciences 104.1 (2007): 36-41.

\bibitem{fortunato2010community}Fortunato, Santo. "Community detection in graphs." Physics reports 486.3 (2010): 75-174.

\bibitem{mckay1981expected}
B. D. McKay. \textit{The expected eigenvalue distribution of a large regular graph. Linear Algebra Appl.,} (1981)

\bibitem{newman2016community} M. E. J. Newman \textit{Community detection in networks: Modularity optimization and maximum likelihood are equivalent.} arXiv preprint arXiv:1606.02319 (2016).

\bibitem{newman2006structure}M. E. J. Newman, A. L. Barabasi, and D. J. Watts.
\textit{The structure and dynamics of networks.} Princeton University
Press, 2006.

\bibitem{barabasi1999emergence}A. L. Barabasi, and R. Albert. \textit{Emergence
of scaling in random networks.} science 286, no. 5439 (1999): 509-512.

\bibitem{buldyrev2010catastrophic}S. V. Buldyrev, R. Parshani, G. P., H. E. Stanley,
and Shlomo Havlin. \textit{Catastrophic cascade of failures in interdependent
networks.} Nature 464, no. 7291 (2010): 1025-1028.

\bibitem{martin2014localization} T. Martin, X. Zhang, and M. E. J. Newman, \textit{Localization
and centrality in networks}, Phys. Rev. E 90, 052808 (2014)

\bibitem{boyd2006computing}S. P. Boyd, P. John , J. F. William, and R. J. Beck.
\textit{Computing core/periphery structures and permutation tests
for social relations data}. Social networks 28, no. 2 (2006): 165-178.

\bibitem{nadakuditi2002graph} R.R. Nadakuditi, M.E.J. Newman, \textit{Graph spectra
and the detectability of community structure in networks}. Phys Rev
Lett 108(18):188701 (2002)

\bibitem{karrer2011stochastic}B. Karrer, M.E.J. Newman, \textit{Stochastic blockmodels
and community structure in networks} Physical Review E 83, 016107,
(2011)

\bibitem{decelle2011asymptotic}A. Decelle, F. Krzakala, C. Moore, L. Zdeborová, \textit{Asymptotic
analysis of the stochastic block model for modular networks and its
algorithmic applications}, Physical Review E, 84,066106, (2011)

\bibitem{chung2003eigenvalues}F. Chung, L. Lu, V. Vu, \textit{Eigenvalues of random
power law graphs} Annals of Combinatorics, (2003).

\bibitem{newman2001random} M.E.J. Newman, S.H. Strogatz, D.J. Watts, \textit{Random
graphs with arbitrary degree distributions and their applications},
Physical review E, Phys. Rev. E 64, 026118 (2001)

\bibitem{zhang2015identification}X. Zhang, T. Martin, M. E. J. Newman. \textit{Identification
of core-periphery structure in networks}. Phys. Rev. E 91, 032803
(2015).

\bibitem{decelle2011inference}A. Decelle, F. Krzakala, C. Moore, L. Zdeborová \textit{Inference
and Phase Transitions in the Detection of Modules in Sparse Networks},
Phys. Rev. Lett. 107, 065701 (2011)

\bibitem{strang2009introduction} G. Strang, \textit{Introduction to Linear Algebra},
Wellesley Cambridge Press, Wellesley, MA, (2009)

\bibitem{borgatti2000models} S. P. Borgatti, P. Stephen, and M. G. Everett. \textit{Models
of core/periphery structures}. Social networks 21, no. 4 (2000): 375-395.

\bibitem{everett1999centrality}M. G. Everett, G. Martin, and S. P. Borgatti. \textit{ The
centrality of groups and classes}. The Journal of mathematical sociology
23, no. 3 (1999): 181-201.

\bibitem{krzakala2013spectral} F. Krzakala, C. Moore, E. Mossel, J. Neeman,
A. Sly, L. Zdeborova, P. Zhang, \textit{Spectral redemption in clustering
sparse networks}. Proc. Natl. Acad. Sci. USA 110 20935-20940 (2013).

\bibitem{Krivelevich2003largest} M. Krivelevich, B. Sudakov , \textit{The largest
eigenvalue of sparse random graphs}. Combin Probab Comput12(01):61-72
(2003)

\bibitem{erdos2013spectral} L. Erdos, A. Knowles, H. Yau, and J. Yin, \textit{Spectral
statistics of Erdos-Renyi graphs I: Local semicircle law}, Ann. Probab.
Volume 41, Number 3B (2013), 2279-2375.

\bibitem{brito2016recovery} Brito, Gerandy, et al. \textit{Recovery and rigidity in a regular stochastic block model.} Proc. of the Twenty-Seventh Annual ACM-SIAM Symposium on Discrete Algorithms. Society for Industrial and Applied Mathematics, 2016.

\bibitem{dumitriu2012sparse}Dumitriu, Ioana, and Soumik Pal. "Sparse regular random graphs: spectral density and eigenvectors." The Annals of Probability 40.5 (2012): 2197-2235.

\bibitem{farkas2001spectra} I. J. Farkas, I. Derenyi, A.L. Barabasi, T. Vicsek,
\textit{Spectra of real-world graphs: Beyond the semicircle law}.
Phys. Rev. E 64, 026704 (2001)

\bibitem{ermann2013spectral} L. Ermann, K. Frahm, and D. Shepelyansky,\textit{Spectral
properties of Google matrix of Wikipedia and other networks}, The
European Physical Journal B 86, 193 (2013)

\bibitem{peixoto2013parsimonious} P.T. Peixoto, \textit{Parsimonious module inference
in large networks}, Physical review letters 110, 14: 148701 (2013)

\bibitem{kawamoto2015limitations}Kawamoto, Tatsuro, and Yoshiyuki Kabashima. "Limitations in the spectral method for graph partitioning: Detectability threshold and localization of eigenvectors." Physical Review E 91.6 (2015): 062803.

\bibitem{rombach2014coreperiphery}M.P. Rombach, A. Mason, J. H. F. Porter, P. J. Mucha.
\textit{Core-periphery structure in networks. } SIAM Journal on Applied
mathematics 74, no. 1 (2014): 167-190.
